GlobalWoZ: Globalizing MultiWoZ to Develop Multilingual Task-Oriented Dialogue Systems

Much recent progress in task-oriented dialogue (ToD) systems has been driven by available annotation data across multiple domains for training. Over the last few years, there has been a move towards data curation for multilingual ToD systems that are applicable to serve people speaking different languages. However, existing multilingual ToD datasets either have a limited coverage of languages due to the high cost of data curation, or ignore the fact that dialogue entities barely exist in countries speaking these languages. To tackle these limitations, we introduce a novel data curation method that generates GlobalWoZ -- a large-scale multilingual ToD dataset globalized from an English ToD dataset for three unexplored use cases. Our method is based on translating dialogue templates and filling them with local entities in the target-language countries. We release our dataset as well as a set of strong baselines to encourage research on learning multilingual ToD systems for real use cases.

==> 05_analysis.tex <==
\section{Future Work}
\label{sec:analysis}
\subsection{Scale up to 20 languages}
The coverage of languages of the existing datasets are still limited to less than 10 languages due to the high cost of data annotation. With our proposed cost-effective data curation method, it is possible to extend the dataset to cover more languages. Thus, we conduct the experiments by evaluating the model performance of our proposed methods (\secref{sec:methodology}) on two sets of test data: (1) \textbf{MT} test data created by machine translation only~(\secref{sec:translate}); (2) \textbf{MTPE} test data first translated by machines and post-edicted later by professional translators. As shown in Table~\ref{tb:f2f_mt_result} and Table~\ref{tb:f2e_mt_result}, the overall reported results on MT test data are higher than those reported on MTPE test data, which is expected because the distribution of the MT test data is more similar to the MT training data. Although there are some differences on individual languages, the conclusions derived from the evaluations on the MT test data remain the same as those derived from the evaluation on the MTPE test data. We also calculate the Spearman rank correlation coefficient and Pearson correlation coefficient between the results on the average results reported on MTPE test data and MT test data in Table~\ref{tb:spearman}, which show a statistically high correlation between the system performance on the MT test data and MTPE test data. Therefore, we show that the MT test data can be used as a proxy to estimate the model performance on the real test data for more languages. We select 20 languages that are supported by Google Translate, Trip Advisor and Booking.com at the same time,  as stated in Table~\ref{tb:selected_languages} in Appendix. We leave the extension of the language coverage to all these languages in our future work. 


\begin{table}[ht!]
\centering
\scalebox{0.75}{
\begin{tabular}{lcccc}
\toprule
\textbf{Methods}           & \textbf{zh} & \textbf{es}  & \textbf{id} &\textbf{avg}\\
\midrule
\notationa         & 1.19  & 1.40  & 1.28  & 1.29  \\
\notationb         & 2.50  & 2.81  & 5.81  & 3.71  \\
\notationc         & 37.79 & 26.95 & 42.59 & 35.78 \\
\notationd         & 38.62 & 27.34 & 42.96 & 36.31 \\
\notatione         & \textbf{39.11} & \textbf{29.17} & 45.39 & 37.89 \\
\notationf         & 38.16 & 29.09 & \textbf{46.51} & \textbf{37.92} \\
\bottomrule
\end{tabular}
}
\caption{Zero-Shot Cross Lingual Joint Accuracy on DST on Target Languages On Use Case F2F - MT test data}
\label{tb:f2f_mt_result}
%\vspace{-1em}
\end{table}


\begin{table}[ht!]
\centering
\scalebox{0.75}{
\begin{tabular}{lcccc}
\toprule
\textbf{Methods}   & \textbf{zh} & \textbf{es}  & \textbf{id} &\textbf{avg}\\
\midrule
\notationa         & 7.61  & 11.67 & 9.64  & 9.64  \\
\notationb         & 2.25  & 5.25  & 5.03  & 4.17  \\
\notationc         & 57.10 & 55.70 & 55.64 & 56.15 \\
\notationd         & 59.05 & \textbf{57.68} & 56.80 & 57.84 \\
\notatione         & \textbf{60.48} & 57.04 & \textbf{58.23} & \textbf{58.76} \\
\notationf.        & 59.21 & 57.51 & 56.41 & 57.71 \\
\bottomrule
\end{tabular}
}
\caption{Zero-Shot and Few-Shot Cross Lingual Joint Accuracy on DST on Target Languages on Use Case F2E - MT test data}
\label{tb:f2e_mt_result}
%\vspace{-1em}
\end{table}


\begin{table}[ht!]
\centering
\scalebox{0.75}{
\begin{tabular}{lcc}
\toprule
\textbf{Methods}          &  \textbf{Spearman Correlation} & \textbf{Pearson Correlation} \\
\midrule
F2F                       &     1.00        &  1.00            \\
F2E                       &     1.00        &  1.00       \\
\bottomrule
\end{tabular}
}
\caption{Spearman Rank Correlation Coefficient between the results on MTPE test data and MT test data}
\label{tb:spearman}
%\vspace{-1em}
\end{table}

\subsection{Few-Shot Cross-lingual Transfer}
Few-shot cross-lingual transfer has attracted lots of research interests recently from both academia and industry. In the few-shot cross-lingual transfer setting, we aim to include a small set of high-quality training data post-edited by professional translators (\secref{sec:translate}) in a target language. This setting is useful to evaluate the efficiency of a multilingual ToD on learning from a small set of target-language data. 


% There is a interesting comparison that we are interested in is the comparison of the task difficulty between a localized dataset and its unlocalized counterpart. With our created template, the comparison can be easily done by replacing the localized ontologies with the unlocalized ontologies, which is purely translated from the English ontologies. 

% \ding{1. Localized Train Set vs Pure MT Train Set and Evaluate on Localized Test Set 2. Localized Train Set evaluate on Localized Test Set vs Pure MT test set}

% \ding{Only DST results}

% \subsection{Localized MT vs Pure MT}
% \label{sec:analysis}
% There is a interesting comparison that we are interested in is the comparison of the task difficulty between a localized dataset and its unlocalized counterpart. With our created template, the comparison can be easily done by replacing the localized ontologies with the unlocalized ontologies, which is purely translated from the English ontologies. 

% \ding{1. Localized Train Set vs Pure MT Train Set and Evaluate on Localized Test Set 2. Localized Train Set evaluate on Localized Test Set vs Pure MT test set}

% \ding{Only DST results}

% \subsection{Scale up to another 3 Languages}

% \ding{lower priority}
% \ding{MT test vs MTPE test to show the ranking is the same}
% Finally, we use MT to create noisy train/dev/test set in another 20 languages to support future research and development of multilingual ToD system. We follow the methods in Section~\ref{sec:methodology} via Machine Translation only without involving any human efforts. The noisy data simulates a baseline for a reasonable scale of languages and can be post edited to become high quality labelled data in the future.



% \begin{table}[ht!]
% \centering
% \scalebox{0.8}{
% \begin{tabular}{lccccccc}
% \toprule
% \textbf{Settings}          & \textbf{zh} & \textbf{es}  & \textbf{id} & \textbf{fr} & \textbf{ja} & \textbf{vi} &\textbf{avg}\\
% \midrule
% Pure Zero-shot \\
% MT + Localization          &               &                \\         
% \bottomrule
% \end{tabular}
% }
% \end{table}
% \ding{Only DST results}


==> 06_conclusion.tex <==
\section{Conclusions}
\label{sec:conclusion}
In this paper, we provide an analysis on three unexplored use cases for multilingual task-oriented dialogue systems. We propose a new data curation method that leverages a machine translation system and local entities in target languages to create a new multilingual TOD dataset -- \name. We propose a series of popular baseline methods and conduct extensive experiments on \name to encourage future research for multilingual ToD systems. %We will continue to develop this dataset to support more languages to benefit the research community. 


\section*{Acknowledgements}
\label{sec:acknowledgements}

%\vspace{-0.5em}
This research is partly supported by the Alibaba-NTU Singapore Joint Research Institute, Nanyang Technological University. We would like to thank the help from our Alibaba colleagues, Ruidan He, Haiyun Peng and Zifan Xu in this work as well. 
